Challenges and Opportunities for Beyond-5G Wireless Security

The demand for broadband wireless access is driving research and standardization of 5G and beyond-5G wireless systems. In this paper, we aim to identify emerging security challenges for these wireless systems and pose multiple research areas to address these challenges.

==> NextG Security/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> NextG Security/programmable-networks.tex <==
\subsection{Programmable Networks} \label{formal}
Many of the above challenges are closely related to the programmable capabilities of modern networks. In particular, network properties like flexibility and adaptability result from the increasing ability of operators to directly program network elements in real time. This softwarization of networks is resulting in large attack surfaces, variable network behavior, and complex protocols and equipment which can be exploited by adversaries.
 
%It is no surprise that similar challenges have been faced during the design of other programmable systems, e.g., in cloud computing. Several important lessons and design principles have come out of the study of these systems. For the next generation of wireless networks, security research can leverage these principles to help address the stated challenges. We now touch upon some of these concepts of programmable systems such as disaggregation, openness and formal methods in the context of wireless systems. 

\textbf{Closing the Security Control Loop:}
Beyond 5G networks will require unprecedented visibility into and control over network behavior to handle their growing security challenges. Such capabilities are needed to quickly identify and respond to evolving threats. Today's mobile networks, however, are not yet able to deliver these security capabilities. This is in part due to the proprietary status of RAN components which are complex, opaque, and difficult to update. 
 
Meanwhile, 5G has begun to adopt concepts like disaggregation and openness for customization and control of network services. %The drive for this adoption has not been led by the security community, but instead by others calling for increasing performance and functionality of wireless networks. To avoid security from becoming a fringe theme in the application of these concepts, security research must embrace disaggregation and openness, and play a larger role in guiding their adoption. In particular, disaggregation can make networks more flexible and thus easier to control. 
With disaggregation, a large complex bundle of network elements is broken up into easier-to-manage pieces. These pieces are often built from commodity hardware that can be directly programmed. In the next generation, disaggregation can enable networks to react quickly to evolving threats.

To illustrate this idea, we can consider the role of disaggregation in SDN. The SDN architecture, illustrated in Fig. \ref{fig:control_loop}, disaggregates the control and data planes, allowing an SDN controller to be placed logically above the data plane for centralized control of commodity switches. As a result of this placement, the controller is strategically positioned for visibility of all network flows. This visibility can be shared with security applications sitting above the controller, which in turn can request the controller to make security-related updates in the data plane. Hence, SDN security applications are well equipped to monitor, analyze, and reprogram the network.
 
In contrast to the above example, networks today monitor and update separately. Updating the network configuration in reaction to security events is made by an open-loop system uses little to no real-time feedback from network monitoring and requires significant human intervention. Hence, security update control is slow to respond to new threats. To address the stated challenges, beyond 5G networks must close the security control loop. The idea of closed-loop network management (often referred to as the ``self-driving network'') has gained a lot of traction in the networking community~\cite{jen-nick:sdn18,srn-report19}.
% juniper-sdn,google:zero-touch, srn-report18, ,Geng2017
Research into self-driving networks is currently in the early stages, and efforts are needed to address the challenges unique to realizing a self-driving RAN. Compared to the core network, a RAN requires more comprehensive monitoring and control due to fast-changing channel conditions and limited bandwidth availability. %\cite{Janakaraj2020}.

A self-driving network for 5G RAN entails the following tasks: (i)~detailed and continuous monitoring of the state of the network, (ii)~making accurate inference decisions in (near) real-time about a myriad of different security events, and (iii)~effective and fast mitigation of each of these events. Realizing these tasks for 5G's RAN entails processing TBs of highly diverse and semantically rich data every second, which in effect rules out the use of off-the-shelf network telemetry tools and network streaming analytics systems~\cite{sonata-paper,univmon}.
% marple-paper
Thus, closing the security loop for the 5G network requires developing an intelligent and resilient network telemetry stack. This stack should make the best use of limited and heterogeneous data plane resources to realize multiple concurrent network analytics tasks, including tasks requiring learning-based inference decisions. 

Developing such a telemetry stack requires interdisciplinary research efforts requiring networking, machine learning, and computer architecture expertise. We envision a ``layered" design, with a middle layer interfacing with a top layer that focuses on ``AI/ML for networking" and a bottom layer concerned with ``networking for AI/ML". The top layer will require the development of reinforcement learning (RL) frameworks responsible for coordinating the execution of a given set of concurrent analytics tasks in ways that best use a given set of hardware targets. The middle layer will serve as ``glue" between the top and bottom layers of the proposed telemetry stack with new learning-based algorithms specifically designed to determine effective query plans that ensure robustness to changes in input traffic and query workload. The bottom layer will require the development of custom hardware targets that are architected specifically with network analytics in mind---enabling flexible analytics tasks dynamically at scale. 


 
 
  \begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{./images/control_loop.pdf}
    \caption{The security control loop. Network state data is collected by devices in the data plane, aggregated at the control plane, and exposed to security applications sitting above the control plane. In turn, these applications can analyze the data and recommend policy changes to the SDN controller. Policy changes are implemented by the SDN controller by reprogramming the data plane.}
    \label{fig:control_loop}
  \end{figure}
 
\textbf{Open RAN:} Comprehensive monitoring and control has been a challenge for RAN operators. In principle, operators should readily be able to collect and aggregate security-relevant data from components across the RAN. Such data should inform the operator on how to tune the right ``control knobs'' and drive the network to a secure state. In practice, monitoring and control is limited by the proprietary status of many components and their interfaces.

Recent standardization efforts like O-RAN %\cite{oran}
have begun to improve monitoring and control by allowing interoperability of RAN components made by different vendors. Interoperability is enabled by opening a number of interfaces between RAN components that were previously vendor-specific, which exposes network state information formerly hidden inside components. For security research, this exposure presents an opportunity for more comprehensive network monitoring and control.

By opening interfaces, we can expect that an O-RAN network will generate ever more security-relevant data from across the network. Combined with the programmability of the network, each switch, gate, controller, and access point can be viewed as a sensor capable of accurately measuring the network state in its locality. Each sensor can be directly programmed via its commodity hardware to report state information back to the operator. Hence, the operator can dynamically tailor each report to contain data as specific and fine-grained as needed. 

Lastly, there are still many open research opportunities for securing the O-RAN architecture itself. There are ongoing concerns that the combining of components from different vendors can lead to security issues. Also, open interfaces present a new attack surface that must be secured. Comprehensive research efforts are needed to address these issues.
 
\textbf{A Formal Approach to Mobile Security:} 
Today, most wireless communications research is focused on adding network functionality and increasing performance. Security is often treated as a second priority behind these two primary objectives. The challenges at hand require a new approach to wireless networking research where functionality/performance is optimized subject to security guarantees.  

Modeling such guarantees requires a formal approach to security. Formal methods will adopt a mathematical framework which allows a protocol designer to precisely describe security goals in the form of formal specifications. Given a mathematical framework, software tools can be used to systematically prove protocol properties and verify that the goals have been met. Most importantly, these tools will allow this to be done without relying on heuristic or ad hoc approaches that can lead to unexpected specification violations. 

Decades of research in networking have produced a number of mature formal tools that are ready to use, yet the application of these tools for wireless security faces a number of challenges. One major challenge is the immense difficulty in extracting formal specifications from the mobile standards, as 5G standards contain informal specifications that are written informally and thus may have different interpretations to different developers. Hence, before formal tools can be applied, these ambiguities must be resolved. Resolving these ambiguities, however, requires a large amount of effort from researchers with a wide-reaching expertise in formal methods, the specifications, and implementation.
 
The value-add from such legwork in formalization will be substantial, as demonstrated by recent standards contributions. Following the release of 5G security specifications in 2018, a small, but growing, body of research has extracted formal specifications for the analysis of 5G security protocols. A few important successes have come out of this work. For instance, vulnerabilities were discovered in the non-access stratum (NAS) and radio resource control (RRC) layer procedures \cite{Hussain2019}. %[6]
These vulnerabilities were inherited from 4G and thus have laid dormant in production deployments for years. 


\rv{The above example illustrates the potential for formal methods to foster trust in wireless security protocols. While the 5G standard is now complete, work will soon begin on the 6G standard, raising opportunities to incorporate formal security requirements and analysis during the pre-release phase of 6G standardization. In particular, 3GPP can better work with the research community to catch security vulnerabilities before the standard is released. Such opportunities can only be realized if closer relationships are fostered between standardization bodies and formal methods researchers.}

% See ``Reactive and Proactive Standardisation of TLS''


Lastly, before formal methods can be integrated into the standards, the community must answer an important question: \textit{how formal should the standards be?} While more formalization allows for stronger security guarantees, formal specifications can also hinder innovation. %Extracting formal specifications from informal standards can be time consuming, dragging out an already slow standardization process. Additionally, gaps in the standard which are now left open to different implementation possibilities will necessarily be closed by formalization. 
In the past, gaps in the standard have been a rich space for innovation, allowing manufacturers and operators to compete by offering better and differentiated products. It is up to the networking community to decide how to balance the above tradeoff between the innovation offered by the current standardization process and security guarantees offered by more formalized specifications. 
%\cgb{this statement is a bit broad. maybe the tradeoff is between having security guarantees from the start, which makes innovation harder, vs. more flexibility for innovation, in which case security guarantees do not come until the standard is stabilized?}.



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
